DreamBooth3D: Subject-Driven Text-to-3D Generation

We present DreamBooth3D, an approach to personalize text-to-3D generative models from as few as 3-6 casually captured images of a subject. Our approach combines recent advances in personalizing text-to-image models (DreamBooth) with text-to-3D generation (DreamFusion). We find that naively combining these methods fails to yield satisfactory subject-specific 3D assets due to personalized text-to-image models overfitting to the input viewpoints of the subject. We overcome this through a 3-stage optimization strategy where we jointly leverage the 3D consistency of neural radiance fields together with the personalization capability of text-to-image models. Our method can produce high-quality, subject-specific 3D assets with text-driven modifications such as novel poses, colors and attributes that are not seen in any of the input images of the subject.

==> bib_long.tex <==
@STRING{CVPR = {Proc. IEEE Conf. on Computer Vision and Pattern	Recognition (CVPR)}}
@STRING{EMMCVPR = {Energy Minimization Methods in Computer Vision and Pattern Recognition (EMMCVPR)}}
@STRING{CVPRWORK = {Proc. IEEE Conf. on Computer Vision and Pattern	Recognition (CVPR) Workshops}}
@STRING{ECCV = {Proc. of the European Conf. on Computer Vision (ECCV)}}
@STRING{ECCVWORK = {Proc. of the European Conf. on Computer Vision (ECCV) Workshops}}
@STRING{ICCV = {Proc. of the IEEE International Conf. on Computer Vision (ICCV)}}
@STRING{ICCVWORK = {Proc. of the IEEE International Conf. on Computer Vision (ICCV) Workshops}}
@STRING{ACCV = {Proc. of the Asian Conf. on Computer Vision (ACCV)}}
@STRING{ACCVWORK = {Proc. of the Asian Conf. on Computer Vision (ACCV) Workshops}}
@STRING{SCIA = {Scandinavian Conference on Image Analysis (SCIA)}}
@STRING{IVCNZ = {Proc. of International Conf. on Image and Vision Computing New Zealand (IVCNZ)}}
@STRING{WACV = {Proc. of the IEEE Winter Conference on Applications of Computer Vision (WACV)}}
@STRING{CVWW = {Proc. of the Computer Vision Winter Workshop (CVWW)}}
@STRING{ISA = {Proc. of the ISPRS Workshop on Image Sequence Analysis (ISA)}}
@STRING{EUROCAST = {Proc. of the International Conf. on Computer Aided Systems Theory (EUROCAST)}}
@STRING{NIPS = {Advances in Neural Information Processing Systems (NIPS)}}
@STRING{NEURIPS = {Advances in Neural Information Processing Systems (NeurIPS)}}
@STRING{NIPSWORK = {Advances in Neural Information Processing Systems (NIPS) Workshops}}
@STRING{NEURIPSWORK = {Advances in Neural Information Processing Systems (NeurIPS) Workshops}}
@STRING{NEURIPSDATA = {Proc. of the Neural Information Processing Systems (NeurIPS) Track on Datasets and Benchmarks}}
@STRING{AISTATS = {Conference on Artificial Intelligence and Statistics (AISTATS)}}
@STRING{JMLR = {Journal of Machine Learning Research (JMLR)}}
@STRING{PAMI = {IEEE Trans. on Pattern Analysis and Machine Intelligence (PAMI)}}
@STRING{CMVP = {Computational Models of Visual Processing}}
@STRING{IJCV = {International Journal of Computer Vision (IJCV)}}
@STRING{JMIV = {Journal of Mathematical Imaging and Vision  (JMIV)}}
@STRING{PR = {Pattern Recognition}}
@STRING{PRL = {Pattern Recognition Letters}}
@STRING{DAGM = {Proc. of the DAGM Symposium on Pattern Recognition (DAGM)}}
@STRING{GCPR = {Proc. of the German Conference on Pattern Recognition (GCPR)}}
@STRING{SI3D = {Proc. of the Symposium on Interactive 3D Graphics (SI3D)}}
@STRING{CVS = {Computer Vision Systems}}
@STRING{ESRT = {Proc. of the Eurographics Symposium on Rendering Techniques (ESRT)}}
@STRING{BMVC = {Proc. of the British Machine Vision Conf. (BMVC)}}
@STRING{PCS = {Proc. of the Picture Coding Symposium (PCS)}}
@STRING{CAIP = {Proc. of the International Conf. on Computer Analysis of Images and Patterns (CAIP)}}
@STRING{SSVM = {Proc. of the International Conf. on Scale Space and Variational Methods in Computer Vision (SSVM)}}
@STRING{ICM = {Proc. of the International Conf. on Multimedia (ICM)}}
@STRING{IUW = {Image Understanding Workshop (IUW)}}
@STRING{ICML = {Proc. of the International Conf. on Machine learning (ICML)}}
@STRING{ICMLWORK = {Proc. of the International Conf. on Machine learning (ICML) Workshops}}
@STRING{ICLR = {Proc. of the International Conf. on Learning Representations (ICLR)}}
@STRING{BN = {Bayesian Nonparametrics (BN)}}
@STRING{CVIU = {Computer Vision and Image Understanding (CVIU)}}
@STRING{JRTIP = {Journal of Real-Time Image Processing (JRTIP)}}
@STRING{ICIP = {Proc. IEEE International Conf. on Image Processing (ICIP)}}
@STRING{JISE = {Journal of Information Science and Engineering (JISE)}}
@STRING{MVA = {Machine Vision and Applications (MVA)}}
@STRING{ICPR = {Proc. of the International Conf. on Pattern Recognition (ICPR)}}
@STRING{ICVS = {Proc. of the International Conf. on Computer Vision Systems (ICVS)}}
@STRING{ICASSP = {Proc. IEEE Conf. on Acoustics, Speech and Signal Processing (ICASSP)}}
@STRING{ITSC = {Proc. IEEE Conf. on Intelligent Transportation Systems (ITSC)}}
@STRING{ITSM = {Proc. IEEE Intelligent Transportation Systems Magazine (ITSM)}}
@STRING{IV = {Proc. IEEE Intelligent Vehicles Symposium (IV)}}
@STRING{IVWORK = {Proc. IEEE Intelligent Vehicles Symposium (IV) Workshops}}
@STRING{IS = {Intelligent Systems (IS)}}
@STRING{TITS = {IEEE Trans. on Intelligent Transportation Systems (TITS)}}
@STRING{SIGGRAPH = {ACM Trans. on Graphics}}
@STRING{TOG = {ACM Trans. on Graphics}}
@STRING{EUROGRAPHICS = {EUROGRAPHICS}}
@STRING{EGSR = {EUROGRAPHICS Symposium on Rendering}}
@STRING{TVC = {The Visual Computer}}
@STRING{TVCG = {IEEE Transactions on Visualization and Computer Graphic (TVCG)}}
@STRING{CGIP = {Computer Graphics and Image Processing (CGIP)}}
@STRING{SGP = {Eurographics Symposium on Geometry Processing (SGP)}}
@STRING{VCG = {IEEE Trans. on Visualization and Computer Graphics (VCG)}}
@STRING{ICRA = {Proc. IEEE International Conf. on Robotics and Automation (ICRA)}}
@STRING{ICRAWORK = {Proc. IEEE International Conf. on Robotics and Automation (ICRA) Workshops}}
@STRING{ACRA = {Proc. IEEE Australasian Conf. on Robotics and Automation (ACRA)}}
@STRING{IROS = {Proc. IEEE International Conf. on Intelligent Robots and Systems (IROS)}}
@STRING{IROSWORK = {Proc. IEEE International Conf. on Intelligent Robots and Systems (IROS) Workshops}}
@STRING{VCIR = {Journal of Visual Communication and Image Representation (VCIR)}}
@STRING{CORL = {Proc. Conf. on Robot Learning (CoRL)}}
@STRING{IJRR = {International Journal of Robotics Research (IJRR)}}
@STRING{JRA = {IEEE Journal of Robotics and Automation (JRA)}}
@STRING{RAL = {IEEE Robotics and Automation Letters (RA-L)}}
@STRING{IJARS = {International Journal of Advanced Robotic Systems (IJARS)}}
@STRING{IAV = {Proc. IFAC Symposium on Intelligent Autonomous Vehicles (IAV)}}
@STRING{ML = {Machine Learning}}
@STRING{TSP = {IEEE Trans. on Signal Processing (TSP)}}
@STRING{SPM = {Signal Processing Magazine}}
@STRING{TIP = {IEEE Trans. on Image Processing (TIP)}}
@STRING{JRSS = {Journal of the Royal Statistical Society (JRSS)}}
@STRING{SAC = {Statistics and Computing}}
@STRING{SS = {Statistical Science}}
@STRING{JASA = {Journal of the American Statistical Association (JASA)}}
@STRING{AAAI = {Proc. of the Conf. on Artificial Intelligence (AAAI)}}
@STRING{THREEDPVT = {International Symposium on 3D Data Processing, Visualization and Transmission (3DPVT)}}
@STRING{THREEDIM = {Proc. of the International Conf. on 3D Digital Imaging and Modeling (THREEDIM)}}
@STRING{THREEDIMPVT = {Proc. of the International Conf. on 3D Digital Imaging, Modeling, Data Processing, Visualization and Transmission (THREEDIMPVT)}}
@STRING{THREEDV = {Proc. of the International Conf. on 3D Vision (3DV)}}
@STRING{IJCAI = {Proc. of the International Joint Conf. on Artificial Intelligence (IJCAI)}}
@STRING{BIOINF = {Bioinformatics}}
@STRING{RAS = {Robotics and Autonomous Systems (RAS)}}
@STRING{AI = {Artificial Intelligence (AI)}}
@STRING{IVC = {Image and Vision Computing (IVC)}}
@STRING{MIA = {Medical Image Analysis (MIA)}}
@STRING{TG = {ACM Trans. on Graphics}}
@STRING{CGF = {Computer Graphics Forum}}
@STRING{CG = {Computers \& Graphics}}
@STRING{TC = {IEEE Trans. on Computers}}
@STRING{TCYB = {IEEE Trans. on Cybernetics}}
@STRING{COMPUTER = {IEEE Computer}}
@STRING{TR = {IEEE Trans. on Robotics}}
@STRING{VISAPP = {Proc. of the Conf. on Computer Vision Theory and Applications (VISAPP)}}
@STRING{AVSS = {Proc. of International Conf. on Advanced Video and Signal Based Surveillance (AVSS)}}
@STRING{ICCEASIA = {Proc. of International Conf. on Consumer Electronics-Asia (ICCE Asia)}}
@STRING{EML = {Encyclopedia of Machine Learning}}
@STRING{IAI = {Proc. IEEE Southwest Symposium on Image Analysis and Interpretation}}
@STRING{RSS = {Proc. Robotics: Science and Systems (RSS)}}
@STRING{ECMR = {Proc. European Conf. on Mobile Robotics (ECMR)}}
@STRING{PCV = {Proc. Photogrammetric Computer Vision (PCV)}}
@STRING{ISVC = {Proc. of the International Symposium on Advances in Visual Computing (ISVC)}}
@STRING{ACVPR = {Advances in Computer Vision and Pattern Recognition (ACVPR)}}
@STRING{LSVGL = {Large-Scale Visual Geo-Localization}}
@STRING{ICANN = {Proc. of the International Conf. on Artificial Neural Networks (ICANN)}}
@STRING{ICAINN = {Proc. of the International Conf. on Artificial Intelligence and Neural Networks (ICAINN)}}
@STRING{ISER = {Proc. of the International Symposium on Experimental Robotics (ISER)}}
@STRING{ISRR = {Proc. of the International Symposium on Robotics Research (ISRR)}}
@STRING{NRLQ = {Naval Research Logistics Quarterly}}
@STRING{ISMAR = {Proc. of the International Symposium on Mixed and Augmented Reality (ISMAR)}}
@STRING{GPGPU = {Proc. of the Workshop on General Purpose Processing on Graphics Processing Units (GPGPU)}}
@STRING{ALMC = {Advances in Large Margin Classifiers}}
@STRING{CPIA = {In ISPRS Conf. Photogrammetric Image Analysis (PIA)}}
@STRING{IIW = {ISPRS Intercommission Workshop}}
@STRING{AVC = {Alvey Vision Conference}}
@STRING{COGIS = {Cognitive Systems with Interactive Sensors (COGIS)}}
@STRING{JIVP = {Journal on Image and Video Processing (JIVP)}}
@STRING{AR = {Autonomous Robots}}
@STRING{ARC = {Annual Reviews in Control}}
@STRING{TRA = {IEEE Trans. on Robotics and Automation (TRA)}}
@STRING{JN = {Journal of Navigation}}
@STRING{RAM = {Robotics and Automation Magazine (RAM)}}
@STRING{JPRS = {ISPRS Journal of Photogrammetry and Remote Sensing (JPRS)}}
@STRING{APRS = {ISPRS Annals of Photogrammetry, Remote Sensing and Spatial Information Sciences (APRS)}}
@STRING{EUROCOLT = {Proc. of European Conf. on Computational Learning Theory (EUROCOLT)}}
@STRING{OE = {Optical Engineering}}
@STRING{SMC = {IEEE Trans. on Systems, Man and Cybernetics (TSMC)}}
@STRING{NC = {Neural Computation}}
@STRING{NN = {Neural Networks}}
@STRING{JOS = {Journal of the Optical Society America (JOSA)}}
@STRING{JBE = {Journal of Basic Engineering (JBE)}}
@STRING{JFR = {Journal of Field Robotics (JFR)}}
@STRING{SIAM = {Journal of the Society for Industrial and Applied Mathematics (SIAM)}}
@STRING{JIS = {Journal of Imaging Sciences (SIAM)}}
@STRING{TAC = {IEEE Trans. on Automatic Control (TAC)}}
@STRING{JCGS = {Journal of Computational and Graphical Statistics (JCGS)}}
@STRING{CGA = {IEEE Computer Graphics and Applications (CGA)}}
@STRING{ACM = {Communications of the ACM}}
@STRING{ARXIV = {arXiv.org}}
@STRING{VMV = {Vision, Modeling and Visualization (VMV)}}
@STRING{NETWORKS = {Networks}}
@STRING{PETS = {Performance Evaluation of Tracking and Surveillance}}
@STRING{CHI = {Proc. of the Conf. on Human Factors in Computing Systems}}
@STRING{FTCGV = {Foundations and Trends in Computer Graphics and Vision}}
@STRING{BC = {Biological Cybernetics}}
@STRING{GPID = {Geometric Properties for Incomplete Data}}
@STRING{MICCAI = {Medical Image Computing and Computer-Assisted Intervention (MICCAI)}}
@STRING{EXPERT = {IEEE Expert}}
@STRING{IFAC = {Proc. of the IFAC Symposium on Intelligent Autonomous Vehicles (IFAC)}}
@STRING{RIC = {Readings in Computer Vision: Issues, Problems, Principles, and Paradigms (RIC)}}
@STRING{AAM = {Advances in Applied Mathematics (AAM)}}
@STRING{SENSORS = {Sensors}}
@STRING{ESA = {Expert Systems With Applications (ESA)}}
@STRING{RRIV = {Registration and Recognition in Images and Videos}}
@STRING{TMI = {The Mathematical Intelligencer}}
@STRING{AMS = {The Annals of Mathematical Statistics}}
@STRING{ESPC = {Proc. of European Signal Processing Conference (ESPC)}}
@STRING{MCNCA = {Multi-Camera Networks: Concepts and Applications (MCNCA)}}
@STRING{ASS = {International Conf. on Advances in System Simulation (ASS)}}
@STRING{Nature = {Nature}}
@STRING{NatureNeuro = {Nature Neuroscience}}
@STRING{PNAS = {Proceedings of the National Academy of Sciences (PNAS)}}
@STRING{PLOSCB = {PLoS Computational Biology (PLOSCB)}}
@STRING{NCNN = {Network: computation in neural systems}}
@STRING{JGT = {Journal of Graphics Tools}}
@STRING{COGSCI = {Proc. of the Annual Meeting of the Cognitive Science Society}}
@STRING{HUMANOIDS = {IEEE-RAS International Conference on Humanoid Robots (Humanoids)}}
@STRING{CVGIP = {Graphical Model and Image Processing (CVGIP)}}
@STRING{ICDAR = {International Conference on Document Analysis and Recognition (ICDAR)}}
@STRING{EICC = {Eurographics Italian Chapter Conference}}
@STRING{IJCNN = {International Joint Conference on Neural Networks (IJCNN)}}
@STRING{ISAMA = {Innovations for Shape Analysis, Models and Algorithms}}
@STRING{FCS = {Frontiers of Computer Science (FCS)}}
@STRING{IECON = {Conference of the {IEEE} Industrial Electronics Society (IECON)}}
@STRING{IECON = {Conference of the {IEEE} Industrial Electronics Society (IECON)}}
@STRING{HPG = {High-Performance Graphics (HPG)}}

